Tumbling Down the Rabbit Hole: How do Assisting Exploration Strategies Facilitate Grey-box Fuzzing?

Many assisting exploration strategies have been proposed to assist grey-box fuzzers in exploring program states guarded by tight and complex branch conditions such as equality constraints. Although they have shown promising results in their original papers, their evaluations seldom follow equivalent protocols, e.g., they are rarely evaluated on identical benchmarks. Moreover, there is a lack of sufficient investigations on the specifics of the program states explored by these strategies which can obfuscate the future application and development of such strategies. Consequently, there is a pressing need for a comprehensive study of assisting exploration strategies on their effectiveness, versatility, and limitations to enlighten their future development. To this end, we perform the first comprehensive study about the assisting exploration strategies for grey-box fuzzers. Specifically, we first collect nine recent fuzzers representing the mainstream assisting exploration strategies as our studied subjects and 21 real-world projects to form our benchmark suite. After evaluating the subjects on the benchmark suite, we then surprisingly find that the dictionary strategy is the most promising since it not only achieves similar or even slightly better performance over the other studied assisting exploration strategies in terms of exploring program states but also is more practical to be enhanced. Accordingly, we propose CDFUZZ, which generates a customized dictionary for each seed upon the baseline fuzzer AFL to improve over the original dictionary strategy. The evaluation results demonstrate that CDFUZZ increases the edge coverage by 16.1% on average for all benchmark projects over the best performer in our study (i.e., AFL++ with the dictionary strategy). CDFUZZ also successfully exposed 37 previously unknown bugs, with nine confirmed and seven fixed by the corresponding developers.

==> figures/const-sym-ratio.tex <==
%auto-ignore
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.98\columnwidth]{figures/SMT-SolvingRate.pdf}
    \caption{The constant-constraints ratio on different benchmarks}
    \label{fig:constraint-ratio}
\end{figure}

==> figures/jhead-iptc.tex <==
%auto-ignore
%@\equal{} fails to be explored by \redqueen{}@escapechar=\@
\begin{figure}[htb]
    \lstset{style=demo-code}
    \centering
    \begin{lstlisting}[language=C, basicstyle={\fontsize{8}{7}\ttfamily}]
void show_IPTC (unsigned char* Data, unsigned int itemlen) {
    const char IptcSig1[] = "Photoshop 3.0";
    const char IptcSig2[] = "8BIM";
    const char IptcSig3[] = {0x04, 0x04};
    unsigned char *pos = Data + sizeof(short);
    // uncovered branch due to failure to locate the offset
    |\uncovered|if (memcmp(pos, IptcSig1, sizeof(IptcSig1)-1) != 0) 
        goto badsig;
    pos += sizeof(IptcSig1);     
    
    if (memcmp(pos, IptcSig2, sizeof(IptcSig2)-1) != 0) 
        goto badsig;
    pos += sizeof(IptcSig2)-1;          

    while (memcmp(pos, IptcSig3, sizeof(IptcSig3)) != 0) {   ...   }
    badsig: 
        ErrNonfatal("IPTC type signature mismatch\n", 0, 0);
    }    \end{lstlisting}
    \caption{An input-to-state fuzzing strategy failure case in \textit{jhead iptc.c}.}
    \label{fig:jhead-memcmp-example}
\end{figure}

==> figures/lou_translate-bug.tex <==
%auto-ignore
%@\equal{} fails to be explored by \redqueen{}@escapechar=\@
\begin{figure}[htb]
    \lstset{style=demo-code}
    \centering
    % \begin{lstlisting}[language=C, basicstyle={\fontsize{8}{7}\ttfamily}]
    \begin{lstlisting}[language=C, basicstyle={\scriptsize\ttfamily}]
while (pos < input->length) {
    |\colorbox{backcolour}{[+] if (pos > 0 \&\& checkCharAttr(...) \&\& ...)}|
            |\colorbox{backcolour}{lastWord = ...; \;\;}|
    switch (transOpcode) {
    case CTO_Literal:
       // pos: 0->1,  3->0
       doCompbrl(..., &pos, ..., &lastWord, ...);
       continue;
    }     ...
    switch (transOpcode) {
    case CTO_Context: 
       // pos: 1->3
       passDoAction(..., &pos, ...);
    }  ...}
    \end{lstlisting}
    \caption{An infinite loop bug in \textit{lou\_translate}}
    \label{fig:liblous-inf-loop}
\end{figure}


% \noindent \textbf{Infinite loop bug in \textit{lou\_translate}.} 
% \approach{} have found an infinite loop bug in \textit{lou\_translate}. The relevant bug issue~\cite{lou-bug-link} has been committed to and fixed by the corresponding developers.

% Figure~\ref{fig:liblous-inf-loop} shows the code snippet that triggered the bug. Line 2 is the entry condition of the infinite loop. In our input, the \codeIn{input->length} is 5. The \codeIn{pos} will be changed in the 2 cases of two switch statements (line 8 and line 14). In the function call of line 8, the `pos` will change from 0 to 1 or from 3 to 0 (the detailed logic is too complicated to describe). In the function call of line 14, the \codeIn{pos} will change from 1 to 3. When an input triggers such an execution track of (line 8, line 14, line 8), it will cause the value of \codeIn{pos} to reciprocate between 0, 1, 3, and 0, always less than \codeIn{input->length}, which will lead to an infinite loop.
% It can be seen that the key to whether fuzzer can easily find such a path lies in whether it can easily enter the two switch-case branches, which is what \approach{} is good at. Its powerful dictionary mechanism can make these two switch cases frequently accessed, thus greatly increasing the probability of triggering the above-mentioned execution track.
 
% In fact, the underlying reason for this bug is quite complicated. The developer fixes this bug by checking and changing some conditions at the beginning of each iteration.

% \noindent \textbf{Infinite loop bug in project \textit{lou\_translate}}. 
% An infinite loop bug was discovered in  \textit{lou\_translate} by \approach{}. The corresponding software developers have successfully resolved the issue as documented in its bug report~\cite{lou-bug-link}. Figure~\ref{fig:liblous-inf-loop} 
% shows the bug-inducing code snippet where the entry condition for the infinite loop is located in line 1. When \codeIn{input->length} equals to 5 in the seed input, variable \codeIn{pos} is updated in two switch statements (lines 7 and 13). Specifically, in the function call of \codeIn{doCompbrl}~\cite{lou-doCompbrl-link} in line 7, the value of \codeIn{pos} is updated from 0 to 1, or from 3 to 0. Similarly, in the function call of \codeIn{passDoAction}~\cite{lou-passDoAction-link} in line 13, \codeIn{pos} is updated from 1 to 3. Thus. the execution path (line 7 $\rightarrow{}$line 13 $\rightarrow{}$line 7) results in looping \codeIn{pos} values $0\rightarrow{}1\rightarrow{}3\rightarrow{}0$. All such values are less than \codeIn{input->length}, i.e., 5, leading to an infinite loop.
% In our evaluation, \approach{} effectively explores the two switch-case branches to expose this bug. 
% In fact, the underlying cause of this bug is relatively complex, and the developer has fixed the issue through rigorous examination and modification of certain conditions (lines 2 to 3) with the following confirmation:

% \devcomment{``I have a fix, which I think will solve the problem properly.''}


% \begin{figure}[htb]
%     \lstset{style=demo-code}
%     \centering
%     \begin{lstlisting}[language=C]
% #define EXIF_JPEG_MARKER JPEG_APP0+1
% #define EXIF_IDENT_STRING "Exif\000\000"
% |\colorbox{backcolour}{[+] \#define EXIF\_IDENT\_STRING\_LEN 6}|
% //...
% while (cmarker) {
%     |\colorbox{uncoveredgray}{[-] if (cmarker->marker == EXIF\_JPEG\_MARKER) \;\;}|
%     |\colorbox{backcolour}{[+] if (cmarker->marker == EXIF\_JPEG\_MARKER \&\&}|
%     |\colorbox{backcolour}{cmarker->data\_length >= EXIF\_IDENT\_STRING\_LEN)}|
%          if (!memcmp(cmarker->data,EXIF_IDENT_STRING,6)) 
% 		          exif_marker=cmarker;
%  	cmarker=cmarker->next;
%  }    \end{lstlisting}
%     \caption{A \hbo{} bug in \textit{jpeginfo}.}
%     \label{fig:jpeginfo-bug}
% \end{figure}
% % |\colorbox{backcolour}{[+] memmove(\&W->Letters[i+1], \&W->Letters[i+2], W->End-i-1);}|


% %@\equal{} fails to be explored by \redqueen{}@escapechar=\@
% \begin{figure}[htb]
%     \lstset{style=demo-code}
%     \centering
%     \begin{lstlisting}[language=C]
% // input->length = 5
% 3630:   
% |\colorbox{uncoveredgray}{[-] while (pos < input->length) \;\;}|
% |\colorbox{backcolour}{[+] while (pos <= input->length) }|
% {
%     |\colorbox{backcolour}{[+] if (pos > 0 \&\&  \;\;}|
%             |\colorbox{backcolour}{[+] checkCharAttr(input->chars[pos - 1], CTC\_Space, table) \&\& \;\;}|
%             |\colorbox{backcolour}{[+] (transOpcode != CTO\_JoinableWord)) \;\;}|
%             |\colorbox{backcolour}{[+] lastWord = ...; \;\;}|
%     |\colorbox{backcolour}{[+] if (pos == input->length) break; \;\;}|
            

% 		  switch (transOpcode) {
% 		      case CTO_Literal:
%                     // pos: 0->1,  3->0
% 3677:               doCompbrl(..., &pos, ..., &lastWord, ...);
%                 //...
%             }
%             switch (transOpcode) {
% 			case CTO_Context: 
%                     // pos: 1->3
% 3747:               passDoAction(..., &pos, ...);
%                 //...
%             }
%         }
% // ...
% }
%     \end{lstlisting}
%     \caption{An infinite loop in \textit{lou\_translate}.}
%     \label{bug:liblous-inf-loop}
% \end{figure}


==> figures/switch_failure_case.tex <==
%auto-ignore
\begin{figure}[htb]
    \lstset{style=demo-code}
    \centering
    \begin{lstlisting}[language=C, basicstyle={\fontsize{8}{7}\ttfamily}]
switch(Format){
|\uncovered|            case FMT_BYTE:      //...
|\uncovered|                break;
            case FMT_SBYTE:
            case FMT_USHORT:
                break;
|\uncovered|            case FMT_SLONG:     //... 
|\uncovered|                break;
            case FMT_URATIONAL: //...
                break;
|\uncovered|            case FMT_SRATIONAL: //...
|\uncovered|                break;
            case FMT_SINGLE:    //...
                break;
|\uncovered|            case FMT_DOUBLE:    //...
|\uncovered|                break;
            default: 
                printf("Unknown format %d:", Format);
                return;
}
    \end{lstlisting}
    \caption{A dictionary fuzzing strategy failure case in \textit{jhead exif.c}}
    \label{fig:switch-failure-case}
\end{figure}



% \begin{figure}[htb]
%     \lstset{style=demo-code}
%     \centering
%     \begin{lstlisting}[language=C]
% switch(Format){
% |\uncovered|            case FMT_BYTE:      //...
% |\uncovered|                break;
%             case FMT_SBYTE:
%             case FMT_USHORT:
%                 break;
% |\uncovered|            case FMT_ULONG:     
% |\uncovered|            case FMT_SLONG:     //... 
% |\uncovered|                break;
% |\uncovered|            case FMT_SSHORT:    //...
% |\uncovered|                break;
%             case FMT_URATIONAL: //...
%                 break;
% |\uncovered|            case FMT_SRATIONAL: //...
% |\uncovered|                break;
%             case FMT_SINGLE:    //...
%                 break;
% |\uncovered|            case FMT_DOUBLE:    //...
% |\uncovered|                break;
%             default: 
%                 printf("Unknown format %d:", Format);
%                 return;
% }
%     \end{lstlisting}
%     \caption{Random dictionary-based fuzzing strategy failure case in \textit{jhead exif.c}\jiahong{The code colored in red is not covered by original random dictionary fuzzing strategy.}}
%     \label{fig:switch-failure-case}
% \end{figure}

==> table/rq2-constaint-slover-dict.tex <==
%auto-ignore
\begin{table*}
    \caption {The edge coverage results of input-to-state and hybrid fuzzers}
    \label{tab:rq2:add-dict-result}
    \setlength\tabcolsep{15pt}
    \begin{adjustbox}{width=0.78\textwidth}
    \begin{tabular}{lrrrrrrrr}
    \hline
    \multirow{2}*{\textbf{Programs}} & \multicolumn{2}{c}{\textbf{\qsym}} & \multicolumn{2}{c}{\textbf{\angora}} & \multicolumn{2}{c}{\textbf{\redqueen}} \\ 
    \cline{2-7}
    &  \textbf{\original} & \textbf{\dictionary}  & \textbf{\original} & \textbf{\dictionary} & \textbf{\original} & \textbf{\dictionary}  \\
    \hline
    
    \bf{readelf}        &  11,386              &  11,524              &  13,291              &  \textbf{14,148}     &  10,053              &  11,432              \\   
    \bf{nm}             &  6,532               &  \textbf{6,573}      &  5,774               &  5,859               &  5,526               &  5,170               \\   
    \bf{objdump}        &  5,999               &  \textbf{6,693}      &  5,863               &  5,939               &  5,587               &  5,884               \\   
    \bf{size}           &  5,211               &  5,215               &  5,201               &  \textbf{5,238}      &  5,002               &  5,012               \\   
    \bf{strip}          &  6,968               &  \textbf{7,144}      &  5,943               &  6,252               &  5,513               &  6,244               \\   
    \bf{djpeg}          &  2,092               &  2,654               &  2,936               &  2,943               &  2,463               &  \textbf{3,007}      \\   
    \bf{tcpdump}        &  10,053              &  10,871              &  9,502               &  10,158              &  11,471              &  \textbf{12,108}     \\   
    \bf{xmllint}        &  6,317               &  \textbf{7,040}      &  4,273               &  6,390               &  6,771               &  7,012               \\   
    \bf{jhead}          &  731                 &  750                 &  157                 &  733                 &  612                 &  \textbf{840}        \\   
    \bf{pngfix}         &  1,976               &  2,001               &  2,161               &  \textbf{2,259}      &  2,189               &  2,237               \\   
    \bf{tiffinfo}       &  3,753               &  4,075               &  4,190               &  4,251               &  3,981               &  \textbf{4,659}      \\   
    \bf{xmlwf}          &  4,797               &  5,074               &  5,132               &  \textbf{5,316}      &  4,879               &  5,050               \\   
    \bf{tiff2bw}        &  2,871               &  3,218               &  3,028               &  3,268               &  3,615               &  \textbf{3,630}      \\   
    \bf{mutool}         &  2,167               &  2,223               &  2,204               &  2,256               &  2,314               &  \textbf{2,349}      \\   
    \hline
    \bf{Average}        &  5,061               &  \textbf{5,361}      &  4,969               &  5,357               &  4,998               &  5,331               \\  
    \textit{p-value}    &   0.005       &       0.005       &       0.005       &       0.005 &       0.005 &       0.005 \\ 
    \hline
    \end{tabular}
    \end{adjustbox}
\end{table*}
 





 

   







==> table/rq3-token-num.tex <==
%auto-ignore
% \begin{table}[]
%     \centering
%     \tiny
%     \caption{Dictionary tokens on each benchmarks}
%     \label{tab:rq3-token-num}
%     \begin{adjustbox}{width=0.88\columnwidth}
%     \begin{tabular}{lcccc}
%     \hline
%     \textbf{Programs} & \textbf{N} & \textbf{M} & \textbf{n }& \textbf{$n/(M \times N)$}\\
%     \hline
% \bf{readelf}        &  2201                &  6330.44             &  83.47               &  5.99 e-6           \\   
% \bf{nm}             &  1234                &  5965.56             &  168.40              &  2.29 e-5            \\   
% \bf{objdump}        &  2289                &  4610.09             &  301.59              &  2.86 e-5            \\   
% \bf{size}           &  1204                &  2966.27             &  93.18               &  2.60 e-5            \\   
% \bf{strip}          &  1453                &  3668.17             &  181.46              &  3.40 e-5            \\   
% \bf{djpeg}          &  155                 &  3358.44             &  4.51                &  8.66 e-5            \\   
% \bf{tcpdump}        &  870                 &  731.48              &  339.91              &  5.34 e-4            \\   
% \bf{xmllint}        &  947                 &  5603.74             &  326.24              &  6.15 e-5            \\   
% \bf{jhead}          &  312                 &  7835.53             &  2.65                &  1.08 e-6            \\   
% \bf{pngfix}         &  285                 &  729.13              &  43.90               &  2.11 e-4            \\   
% \bf{tiffinfo}       &  336                 &  2082.26             &  27.83               &  3.98 e-5            \\   
% \bf{xmlwf}          &  158                 &  1050.74             &  3.63                &  2.18 e-5            \\   
% \bf{tiff2bw}        &  338                 &  13080.78            &  26.52               &  6.00 e-6            \\   
% \bf{mutool}         &  6330                &  6998.70             &  557.17              &  1.26 e-5            \\   
% \hline
% \bf{Average}        &  1294                &  4643.36             &  154.32              &  7.24 e-5            \\  
%     \hline
%     \end{tabular}
%     \end{adjustbox}
% \end{table}

% \begin{table}[]
%     \centering
%     \tiny
%     \caption{Dictionary tokens on each benchmarks}
%     \label{tab:rq3-token-num}
%     \begin{adjustbox}{width=0.88\columnwidth}
%     \begin{tabular}{lccccr}
%     \hline
%     \textbf{Programs} & \textbf{N} & \textbf{M} & \textbf{n} & \textbf{$n/(M \times N)$} & \textbf{$n/M$}\\
%     \hline
% \bf{readelf}        &  2201                &  6330.44             &  83.47               &  5.99 e-6        &       1.32 e-2      \\   
% \bf{nm}             &  1234                &  5965.56             &  168.40              &  2.29 e-5        &       2.82 e-2      \\   
% \bf{objdump}        &  2289                &  4610.09             &  301.59              &  2.86 e-5        &       6.54 e-2      \\   
% \bf{size}           &  1204                &  2966.27             &  93.18               &  2.60 e-5        &       3.14 e-2      \\   
% \bf{strip}          &  1453                &  3668.17             &  181.46              &  3.40 e-5        &       4.95 e-2      \\   
% \bf{djpeg}          &  155                 &  3358.44             &  4.51                &  8.66 e-5        &       1.34 e-3      \\   
% \bf{tcpdump}        &  870                 &  731.48              &  339.91              &  5.34 e-4        &       4.65 e-1      \\   
% \bf{xmllint}        &  947                 &  5603.74             &  326.24              &  6.15 e-5        &       5.82 e-2      \\   
% \bf{jhead}          &  312                 &  7835.53             &  2.65                &  1.08 e-6        &       3.38 e-4      \\   
% \bf{pngfix}         &  285                 &  729.13              &  43.90               &  2.11 e-4        &       6.02 e-2      \\   
% \bf{tiffinfo}       &  336                 &  2082.26             &  27.83               &  3.98 e-5        &       1.33 e-2      \\   
% \bf{xmlwf}          &  158                 &  1050.74             &  3.63                &  2.18 e-5        &       3.45 e-3      \\   
% \bf{tiff2bw}        &  338                 &  13080.78            &  26.52               &  6.00 e-6        &       2.03 e-3      \\   
% \bf{mutool}         &  6330                &  6998.70             &  557.17              &  1.26 e-5        &       7.96 e-2      \\   
% \hline
% \bf{Average}        &  1294                &  4643.36             &  154.32              &  7.24 e-5        &       6.22 e-2      \\  
%     \hline
%     \end{tabular}
%     \end{adjustbox}
% \end{table}


\begin{table}[]
    \centering
    \tiny
    \caption{The probabilities of successful token insertion}
    \label{tab:rq3-token-num}
    \begin{adjustbox}{width=0.88\columnwidth}
    \begin{tabular}{lccccr}
    \hline
    \textbf{Programs} & \textbf{N} & \textbf{M} & \textbf{n} & \textbf{$n/(M \times N)$} & \textbf{$1/M$}\\
    \hline
\bf{readelf}        &  2201                &  6330.44             &  83.47               &  5.99 e-6        &       1.57 e-4      \\   
\bf{nm}             &  1234                &  5965.56             &  168.40              &  2.29 e-5        &       1.68 e-4      \\   
\bf{objdump}        &  2289                &  4610.09             &  301.59              &  2.86 e-5        &       2.17 e-4      \\   
\bf{size}           &  1204                &  2966.27             &  93.18               &  2.60 e-5        &       3.37 e-4      \\   
\bf{strip}          &  1453                &  3668.17             &  181.46              &  3.40 e-5        &       2.72 e-4      \\   
\bf{djpeg}          &  155                 &  3358.44             &  4.51                &  8.66 e-5        &       2.98 e-4      \\   
\bf{tcpdump}        &  870                 &  731.48              &  339.91              &  5.34 e-4        &       1.37 e-3      \\   
\bf{xmllint}        &  947                 &  5603.74             &  326.24              &  6.15 e-5        &       1.78 e-4      \\   
\bf{jhead}          &  312                 &  7835.53             &  2.65                &  1.08 e-6        &       1.28 e-4      \\   
\bf{pngfix}         &  285                 &  729.13              &  43.90               &  2.11 e-4        &       1.37 e-3      \\   
\bf{tiffinfo}       &  336                 &  2082.26             &  27.83               &  3.98 e-5        &       4.80 e-4      \\   
\bf{xmlwf}          &  158                 &  1050.74             &  3.63                &  2.18 e-5        &       9.52 e-4      \\   
\bf{tiff2bw}        &  338                 &  13080.78            &  26.52               &  6.00 e-6        &       7.64 e-5      \\   
\bf{mutool}         &  6330                &  6998.70             &  557.17              &  1.26 e-5        &       1.43 e-4      \\   
\hline
\bf{Average}        &  1294                &  4643.36             &  154.32              &  7.24 e-5        &       4.38 e-4      \\  
    \hline
    \end{tabular}
    \end{adjustbox}
\end{table}
